Unified Interpretation of Smoothing Methods for Negative Sampling Loss Functions in Knowledge Graph Embedding

Knowledge Graphs (KGs) are fundamental resources in knowledge-intensive tasks in NLP. Due to the limitation of manually creating KGs, KG Completion (KGC) has an important role in automatically completing KGs by scoring their links with KG Embedding (KGE). To handle many entities in training, KGE relies on Negative Sampling (NS) loss that can reduce the computational cost by sampling. Since the appearance frequencies for each link are at most one in KGs, sparsity is an essential and inevitable problem. The NS loss is no exception. As a solution, the NS loss in KGE relies on smoothing methods like Self-Adversarial Negative Sampling (SANS) and subsampling. However, it is uncertain what kind of smoothing method is suitable for this purpose due to the lack of theoretical understanding. This paper provides theoretical interpretations of the smoothing methods for the NS loss in KGE and induces a new NS loss, Triplet Adaptive Negative Sampling (TANS), that can cover the characteristics of the conventional smoothing methods. Experimental results of TransE, DistMult, ComplEx, RotatE, HAKE, and HousE on FB15k-237, WN18RR, and YAGO3-10 datasets and their sparser subsets show the soundness of our interpretation and performance improvement by our TANS.

==> inputs/_full_results.tex <==
\begin{table}[htbp]
    \centering
    \caption{Results on FB15k-237.\label{tab:fb15k-237}}
    \resizebox{0.7\columnwidth}{!}{
    \small
    {
    \renewcommand{\arraystretch}{0.835}
    \begin{tabular}{cccccccccccc}
    \toprule
    \multicolumn{12}{c}{FB15k-237} \\
    \midrule
    \multirow{2}[4]{*}{Model} & \multicolumn{2}{c}{Subsampling} & \multicolumn{2}{c}{MRR} & \multicolumn{2}{c}{H@1} & \multicolumn{2}{c}{H@3} & \multicolumn{2}{c}{H@10} & \multirow{1.5}[4]{*}{$\gamma$} \\
\cmidrule{2-11}          & Assumption & Loss  & Mean  & SD    & Mean  & SD    & Mean  & SD    & Mean  & SD    &  \\
    \midrule
    \multirow{12}[23]{*}{ComplEx} & \multirow{2.2}[6]{*}{None} & NS    & 23.9  & 0.2   & 15.8  & 0.1   & 26.1  & 0.3   & 40.0  & 0.2   & \textbf{-} \\
\cmidrule{3-12}          &       & SANS  & 22.3  & 0.1   & 13.8  & 0.1   & 24.2  & 0.0   & 39.5  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{32.8 } & 0.2   & \textbf{23.2 } & 0.1   & \textbf{36.2 } & 0.2   & \textbf{52.2 } & 0.1   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 27.2  & 0.1   & 19.1  & 0.1   & 29.5  & 0.1   & 43.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 32.3  & 0.0   & 23.0  & 0.1   & 35.4  & 0.1   & 51.2  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{33.3 }} & 0.0   & $^{\dagger}${\textbf{23.8 }} & 0.1   & $^{\dagger}${\textbf{36.9 }} & 0.1   & $^{\dagger}${\textbf{52.7 }} & 0.0   & -1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 25.1  & 0.2   & 17.1  & 0.3   & 27.4  & 0.2   & 41.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 32.7  & 0.1   & 23.6  & 0.1   & 36.0  & 0.1   & 51.2  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{33.3 }} & 0.0   & $^{\dagger}${\textbf{23.8 }} & 0.0   & \textbf{36.8 } & 0.1   & \textbf{52.1 } & 0.2   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 22.8  & 0.4   & 14.7  & 0.5   & 24.7  & 0.4   & 39.0  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 32.6  & 0.0   & \textbf{23.5 } & 0.1   & 35.8  & 0.1   & 51.2  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{33.0 } & 0.1   & \textbf{23.5 } & 0.1   & \textbf{36.5 } & 0.1   & \textbf{52.1 } & 0.1   & -0.5 \\
    \midrule
    \multirow{12}[23]{*}{DistMult} & \multirow{2.2}[6]{*}{None} & NS    & 23.3  & 0.1   & 15.6  & 0.1   & 25.7  & 0.1   & 38.4  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 22.3  & 0.1   & 14.0  & 0.2   & 24.1  & 0.1   & 39.2  & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{31.0 } & 0.1   & \textbf{21.7 } & 0.1   & \textbf{34.0 } & 0.1   & \textbf{49.6 } & 0.1   & -1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 25.4  & 0.1   & 17.9  & 0.1   & 27.6  & 0.1   & 40.4  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 30.8  & 0.1   & 21.9  & 0.1   & 33.6  & 0.1   & 48.4  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{31.5 }} & 0.1   & $^{\dagger}${\textbf{22.4 }} & 0.1   & $^{\dagger}${\textbf{34.6 }} & 0.1   & $^{\dagger}${\textbf{49.7 }} & 0.0   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 24.0  & 0.1   & 16.7  & 0.2   & 25.9  & 0.1   & 38.4  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 29.9  & 0.0   & 21.2  & 0.1   & 32.8  & 0.0   & 47.5  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{30.7 } & 0.0   & \textbf{21.6 } & 0.0   & \textbf{34.0 } & 0.0   & \textbf{49.0 } & 0.0   & -1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 21.0  & 0.1   & 13.5  & 0.2   & 22.8  & 0.2   & 36.3  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 29.2  & 0.0   & 20.5  & 0.1   & 31.9  & 0.0   & 46.7  & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{30.7 } & 0.1   & \textbf{21.5 } & 0.1   & \textbf{33.8 } & 0.1   & \textbf{49.3 } & 0.1   & -2 \\
    \midrule
    \multirow{12}[23]{*}{TransE} & \multirow{2.2}[6]{*}{None} & NS    & 30.4  & 0.0   & 21.3  & 0.1   & 33.4  & 0.1   & 48.5  & 0.0   & - \\
\cmidrule{3-12}          &       & SANS  & 33.0  & 0.1   & 22.9  & 0.1   & 37.2  & 0.1   & $^{\dagger}${\textbf{53.0 }} & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{33.6 } & 0.0   & \textbf{23.9 } & 0.0   & \textbf{37.3 } & 0.0   & $^{\dagger}${\textbf{53.0 }} & 0.1   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 29.4  & 0.1   & 20.0  & 0.1   & 32.8  & 0.0   & 48.1  & 0.0   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{33.0 } & 0.1   & 23.1  & 0.1   & \textbf{36.8 } & 0.1   & \textbf{52.7 } & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{33.0 } & 0.0   & 23.1  & 0.0   & \textbf{36.8 } & 0.1   & \textbf{52.7 } & 0.1   & -0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 29.3  & 0.1   & 20.0  & 0.1   & 32.8  & 0.1   & 47.8  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{33.5 } & 0.0   & \textbf{23.9 } & 0.1   & \textbf{37.2 } & 0.1   & \textbf{52.8 } & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{33.5 } & 0.1   & \textbf{23.9 } & 0.1   & \textbf{37.2 } & 0.0   & \textbf{52.8 } & 0.1   & -0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 30.1  & 0.1   & 21.0  & 0.1   & 33.6  & 0.0   & 48.0  & 0.0   & - \\
\cmidrule{3-12}          &       & SANS  & 33.5  & 0.0   & 23.9  & 0.0   & 37.3  & 0.2   & 52.7  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{34.0 }} & 0.1   & $^{\dagger}${\textbf{24.5 }} & 0.1   & $^{\dagger}${\textbf{37.7 }} & 0.1   & $^{\dagger}${\textbf{53.0 }} & 0.1   & 0.5 \\
    \midrule
    \multirow{12}[23]{*}{RotatE} & \multirow{2.2}[6]{*}{None} & NS    & 30.3  & 0.0   & 21.4  & 0.1   & 33.2  & 0.1   & 48.4  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 32.9  & 0.1   & 22.8  & 0.1   & 36.8  & 0.0   & 53.1  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{34.1 } & 0.1   & \textbf{24.6 } & 0.1   & \textbf{37.7 } & 0.1   & $^{\dagger}${\textbf{53.3 }} & 0.1   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 29.5  & 0.0   & 20.3  & 0.0   & 32.7  & 0.1   & 47.9  & 0.0   & - \\
\cmidrule{3-12}          &       & SANS  & 33.6  & 0.1   & 23.9  & 0.1   & 37.3  & 0.1   & \textbf{53.1 } & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{33.8 } & 0.0   & \textbf{24.2 } & 0.0   & \textbf{37.4 } & 0.0   & 53.0  & 0.1   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 29.4  & 0.1   & 20.2  & 0.1   & 32.6  & 0.1   & 47.6  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 34.0  & 0.1   & \textbf{24.6 } & 0.0   & \textbf{37.7 } & 0.0   & 53.0  & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{34.1 } & 0.0   & \textbf{24.6 } & 0.0   & \textbf{37.7 } & 0.0   & \textbf{53.1 } & 0.1   & -0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 30.1  & 0.0   & 21.2  & 0.1   & 33.3  & 0.1   & 47.7  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 33.9  & 0.1   & 24.4  & 0.1   & 37.6  & 0.1   & 52.9  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{34.2 }} & 0.0   & $^{\dagger}${\textbf{24.7 }} & 0.1   & $^{\dagger}${\textbf{37.8 }} & 0.0   & \textbf{53.1 } & 0.1   & 0.5 \\
    \midrule
    \multirow{12}[23]{*}{HAKE} & \multirow{2.2}[6]{*}{None} & NS    & 30.8  & 0.1   & 21.8  & 0.1   & 33.8  & 0.1   & 48.6  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 32.8  & 0.2   & 22.7  & 0.3   & 36.9  & 0.1   & 52.8  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{34.4 } & 0.1   & \textbf{24.9 } & 0.1   & \textbf{37.9 } & 0.2   & \textbf{53.6 } & 0.0   & -0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 30.4  & 0.1   & 21.6  & 0.1   & 33.3  & 0.1   & 48.2  & 0.0   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{34.1 } & 0.1   & \textbf{24.4 } & 0.1   & \textbf{37.9 } & 0.1   & 53.6  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{34.1 } & 0.0   & \textbf{24.4 } & 0.0   & \textbf{37.9 } & 0.0   & \textbf{53.7 } & 0.0   & -0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 30.2  & 0.1   & 21.5  & 0.0   & 33.1  & 0.0   & 47.7  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{34.7 } & 0.0   & \textbf{25.2 } & 0.1   & \textbf{38.2 } & 0.0   & \textbf{53.8 } & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & 34.6  & 0.0   & 25.0  & 0.1   & \textbf{38.2 } & 0.2   & 53.7  & 0.1   & 0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 30.7  & 0.1   & 22.2  & 0.1   & 33.5  & 0.1   & 48.0  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 34.7  & 0.1   & 25.1  & 0.1   & 38.3  & 0.1   & 53.9  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{34.9 }} & 0.0   & $^{\dagger}${\textbf{25.4 }} & 0.0   & $^{\dagger}${\textbf{38.6 }} & 0.1   & $^{\dagger}${\textbf{54.0 }} & 0.1   & 0.5 \\
    \bottomrule
    \end{tabular}}
    }%
\end{table}%


\begin{table}[htbp]
    \caption{Results on WN18RR.\label{tab:wn18rr}}
    \centering
    \resizebox{0.7\columnwidth}{!}{
    \small
    {
    \renewcommand{\arraystretch}{0.6}
    \begin{tabular}{cccccccccccc}
    \toprule
    \multicolumn{12}{c}{WN18RR} \\
    \midrule
    \multirow{2}[4]{*}{Model} & \multicolumn{2}{c}{\multirow{2}[4]{*}{Subsampling}} & \multicolumn{2}{c}{MRR} & \multicolumn{2}{c}{H@1} & \multicolumn{2}{c}{H@3} & \multicolumn{2}{c}{H@10} & \multirow{1.5}[4]{*}{$\gamma$} \\
\cmidrule{4-11}          & \multicolumn{2}{c}{} & Mean  & SD    & Mean  & SD    & Mean  & SD    & Mean  & SD    &  \\
    \midrule
    \multirow{13}[23]{*}{ComplEx} & \multirow{2.2}[6]{*}{None} & NS    & 44.5  & 0.1   & 38.1  & 0.2   & 48.3  & 0.2   & 55.5  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 45.0  & 0.1   & 41.0  & 0.1   & 46.5  & 0.3   & 53.3  & 0.3   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{47.3 } & 0.0   & \textbf{43.3 } & 0.0   & \textbf{49.1 } & 0.1   & \textbf{55.7 } & 0.1   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 45.0  & 0.1   & 38.9  & 0.1   & 48.6  & 0.2   & 55.7  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 46.9  & 0.1   & 42.7  & 0.2   & 48.5  & 0.2   & 55.5  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{47.7 } & 0.2   & \textbf{43.6 } & 0.1   & \textbf{49.3 } & 0.2   & \textbf{55.9 } & 0.3   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 45.1  & 0.1   & 38.9  & 0.1   & 48.8  & 0.2   & 56.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 47.4  & 0.1   & 43.2  & 0.1   & 49.2  & 0.2   & 56.0  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{48.0 } & 0.1   & 43.9  & 0.1   & $^{\dagger}${\textbf{49.7 }} & 0.1   & \textbf{56.1 } & 0.1   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 45.0  & 0.1   & 38.7  & 0.1   & 48.8  & 0.1   & 56.0  & 0.3   & - \\
\cmidrule{3-12}          &       & SANS  & 47.5  & 0.1   & 43.3  & 0.1   & 49.1  & 0.2   & 56.2  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{48.3 }} & 0.1   & $^{\dagger}${\textbf{44.4 }} & 0.2   & 49.6  & 0.1   & $^{\dagger}${\textbf{56.3 }} & 0.2   & -1 \\
    \midrule
    \multirow{13}[23]{*}{DistMult} & \multirow{2.2}[6]{*}{None} & NS    & 38.5  & 0.2   & 30.6  & 0.3   & 42.9  & 0.2   & 52.5  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 42.4  & 0.0   & 38.2  & 0.1   & 43.7  & 0.0   & 51.0  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{44.2 } & 0.1   & \textbf{40.1 } & 0.1   & \textbf{45.3 } & 0.1   & \textbf{53.2 } & 0.2   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 39.3  & 0.2   & 31.9  & 0.2   & 43.3  & 0.1   & 53.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 43.9  & 0.1   & 39.4  & 0.1   & 45.2  & 0.1   & 53.3  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{44.6 } & 0.0   & \textbf{40.5 } & 0.2   & \textbf{45.7 } & 0.1   & \textbf{53.9 } & 0.1   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 39.0  & 0.2   & 31.2  & 0.2   & 43.2  & 0.1   & 52.9  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 44.5  & 0.1   & 40.0  & 0.1   & \textbf{46.0 } & 0.1   & \textbf{54.2 } & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{44.7 } & 0.1   & \textbf{40.5 } & 0.2   & 45.8  & 0.0   & 54.0  & 0.2   & -2 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 38.8  & 0.2   & 30.8  & 0.2   & 43.1  & 0.1   & 53.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 44.7  & 0.1   & 40.1  & 0.1   & $^{\dagger}${\textbf{46.2 }} & 0.3   & 54.3  & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{45.0 }} & 0.1   & $^{\dagger}${\textbf{40.7 }} & 0.1   & 46.1  & 0.2   & $^{\dagger}${\textbf{54.5 }} & 0.2   & -0.5 \\
    \midrule
    \multirow{13}[23]{*}{TransE} & \multirow{2.2}[6]{*}{None} & NS    & 21.1  & 0.0   & 2.1   & 0.1   & 36.5  & 0.2   & 50.4  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 22.5  & 0.1   & 1.7   & 0.1   & \textbf{40.2 } & 0.1   & 52.5  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{22.7 } & 0.0   & \textbf{2.5 } & 0.0   & 39.5  & 0.2   & \textbf{53.4 } & 0.1   & 0.5 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 20.3  & 0.1   & \textbf{1.6 } & 0.1   & 35.1  & 0.2   & 49.9  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 22.3  & 0.0   & 1.3   & 0.1   & \textbf{40.2 } & 0.1   & 52.9  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{22.4 } & 0.1   & 1.4   & 0.1   & 40.1  & 0.1   & \textbf{53.0 } & 0.1   & 0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 21.0  & 0.1   & 1.8   & 0.1   & 36.4  & 0.2   & 51.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 23.0  & 0.0   & 1.9   & 0.1   & 40.9  & 0.2   & 53.6  & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{23.1 } & 0.0   & \textbf{2.1 } & 0.0   & $^{\dagger}${\textbf{41.0 }} & 0.1   & \textbf{53.8 } & 0.0   & 0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 21.5  & 0.1   & 2.2   & 0.0   & 37.2  & 0.1   & 51.4  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 23.2  & 0.0   & 2.3   & 0.1   & \textbf{40.9 } & 0.2   & 53.6  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{23.3 }} & 0.1   & $^{\dagger}${\textbf{3.0 }} & 0.0   & 40.2  & 0.2   & $^{\dagger}${\textbf{54.4 }} & 0.1   & 0.5 \\
    \midrule
    \multirow{13}[23]{*}{RotatE} & \multirow{2.2}[6]{*}{None} & NS    & 47.0  & 0.1   & 42.5  & 0.2   & 48.6  & 0.2   & 55.8  & 0.3   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{47.2 } & 0.1   & \textbf{42.6 } & 0.1   & \textbf{49.1 } & 0.1   & \textbf{56.7 } & 0.0   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{47.3 } & 0.1   & \textbf{42.6 } & 0.1   & \textbf{49.1 } & 0.1   & \textbf{56.7 } & 0.1   & -0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 47.0  & 0.0   & 42.2  & 0.1   & 48.7  & 0.1   & 56.3  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{47.5 } & 0.1   & \textbf{42.7 } & 0.2   & \textbf{49.3 } & 0.1   & \textbf{57.2 } & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{47.5 } & 0.1   & \textbf{42.7 } & 0.2   & \textbf{49.3 } & 0.1   & 57.1  & 0.1   & 0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 47.1  & 0.1   & 42.3  & 0.1   & 48.7  & 0.1   & 56.4  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{47.7 } & 0.1   & $^{\dagger}${\textbf{42.9 }} & 0.2   & 49.6  & 0.0   & \textbf{57.4 } & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{47.7 } & 0.1   & 42.8  & 0.2   & \textbf{49.7 } & 0.1   & \textbf{57.4 } & 0.1   & 0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 47.2  & 0.2   & 42.7  & 0.2   & 48.7  & 0.1   & 56.3  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 47.7  & 0.1   & $^{\dagger}${\textbf{42.9 }} & 0.1   & 49.6  & 0.1   & 57.2  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{47.8 }} & 0.2   & 42.8  & 0.3   & $^{\dagger}${\textbf{49.8 }} & 0.1   & $^{\dagger}${\textbf{57.6 }} & 0.1   & 0.5 \\
    \midrule
    \multirow{13}[23]{*}{HAKE} & \multirow{2.2}[6]{*}{None} & NS    & 48.8  & 0.1   & \textbf{44.5 } & 0.1   & 50.5  & 0.2   & 57.3  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{48.9 } & 0.0   & \textbf{44.5 } & 0.2   & \textbf{50.6 } & 0.3   & 57.7  & 0.1   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{48.9 } & 0.0   & 44.4  & 0.1   & 50.5  & 0.3   & \textbf{57.8 } & 0.1   & 0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 49.2  & 0.0   & 44.6  & 0.1   & 51.1  & 0.1   & 57.9  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{49.5 } & 0.1   & \textbf{45.0 } & 0.2   & 51.2  & 0.2   & 58.2  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{49.5 } & 0.1   & \textbf{45.0 } & 0.2   & 51.2  & 0.3   & \textbf{58.4 } & 0.2   & 0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 49.3  & 0.1   & 44.8  & 0.1   & 51.3  & 0.2   & 58.0  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{49.7 } & 0.1   & \textbf{45.2 } & 0.2   & 51.5  & 0.1   & \textbf{58.4 } & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{49.7 } & 0.0   & \textbf{45.2 } & 0.2   & \textbf{51.6 } & 0.3   & \textbf{58.4 } & 0.2   & -0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 49.4  & 0.2   & 44.9  & 0.2   & 51.3  & 0.2   & 57.8  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & $^{\dagger}${\textbf{49.9 }} & 0.0   & 45.3  & 0.1   & $^{\dagger}${\textbf{51.8 }} & 0.2   & $^{\dagger}${\textbf{58.6 }} & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{49.9 }} & 0.1   & $^{\dagger}${\textbf{45.4 }} & 0.1   & $^{\dagger}${\textbf{51.8 }} & 0.2   & 58.5  & 0.2   & 0.05 \\
    \bottomrule
    \end{tabular}}
    }%
\end{table}%

\begin{table}[htbp]
    \centering
    \caption{Results on YAGO3-10. \label{tab:YAGO3-10}}
    \resizebox{\columnwidth}{!}{
    \small
    {
    \renewcommand{\arraystretch}{0.6}
    \begin{tabular}{cccccccccccc}
    \toprule
    \multicolumn{12}{c}{YAGO3-10} \\
    \midrule
    \multirow{2}[4]{*}{Model} & \multicolumn{2}{c}{\multirow{2}[4]{*}{Subsampling}} & \multicolumn{2}{c}{MRR} & \multicolumn{2}{c}{H@1} & \multicolumn{2}{c}{H@3} & \multicolumn{2}{c}{H@10} & \multirow{1.5}[4]{*}{$\gamma$} \\
\cmidrule{4-11}          & \multicolumn{2}{c}{} & Mean  & SD    & Mean  & SD    & Mean  & SD    & Mean  & SD    &  \\
    \midrule
    \multirow{13}[23]{*}{RotatE} & \multirow{2.2}[6]{*}{None} & NS    & 43.5  & 0.1   & 32.8  & 0.2   & 49.1  & 0.2   & 63.7  & 0.3   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{49.6 } & 0.2   & 39.9  & 0.1   & 55.3  & 0.3   & \textbf{67.3 } & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{49.6 } & 0.2   & \textbf{40.0 } & 0.2   & \textbf{55.4 } & 0.5   & 67.2  & 0.3   & -0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 44.8  & 0.1   & 34.5  & 0.3   & 50.0  & 0.2   & 64.7  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{49.6 } & 0.3   & \textbf{40.1 } & 0.3   & \textbf{55.2 } & 0.4   & \textbf{67.4 } & 0.3   & - \\
\cmidrule{3-12}          &       & T-SANS & 49.5  & 0.3   & \textbf{40.1 } & 0.3   & 55.0  & 0.5   & 67.3  & 0.3   & -0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 44.8  & 0.2   & 34.5  & 0.3   & 50.0  & 0.1   & 64.7  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{49.9 } & 0.2   & \textbf{40.5 } & 0.3   & \textbf{55.5 } & 0.5   & \textbf{67.4 } & 0.3   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{49.9 } & 0.2   & \textbf{40.5 } & 0.3   & \textbf{55.5 } & 0.5   & \textbf{67.4 } & 0.2   & 0.01 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 44.4  & 0.2   & 34.0  & 0.3   & 49.8  & 0.2   & 64.3  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 50.0  & 0.3   & 40.6  & 0.2   & 55.6  & 0.3   & 67.5  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & $^{\dagger}${\textbf{50.1 }} & 0.2   & $^{\dagger}${\textbf{40.7 }} & 0.1   & $^{\dagger}${\textbf{55.7 }} & 0.3   & $^{\dagger}${\textbf{67.6 }} & 0.3   & 0.05 \\
    \midrule
    \multirow{13}[23]{*}{HAKE} & \multirow{2.2}[6]{*}{None} & NS    & 47.4  & 0.3   & 36.6  & 0.5   & 53.9  & 0.1   & 67.0  & 0.1   & - \\
\cmidrule{3-12}          &       & SANS  & 53.5  & 0.2   & 44.6  & 0.3   & \textbf{59.1 } & 0.4   & \textbf{69.0 } & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{53.7 } & 0.1   & \textbf{45.3 } & 0.3   & 59.0  & 0.1   & 68.8  & 0.1   & 0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Base} & NS    & 48.8  & 0.3   & 38.4  & 0.4   & 55.0  & 0.2   & 68.1  & 0.3   & - \\
\cmidrule{3-12}          &       & SANS  & \textbf{54.6 } & 0.2   & \textbf{46.2 } & 0.3   & 59.9  & 0.2   & 69.6  & 0.2   & - \\
\cmidrule{3-12}          &       & T-SANS & 54.5  & 0.2   & 45.9  & 0.3   & 59.9  & 0.2   & \textbf{69.9 } & 0.1   & -0.1 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Freq} & NS    & 49.3  & 0.2   & 39.1  & 0.3   & 55.4  & 0.1   & 68.1  & 0.2   & - \\
\cmidrule{3-12}          &       & SANS  & 54.6  & 0.4   & 46.0  & 0.7   & \textbf{60.2 } & 0.1   & \textbf{69.6 } & 0.3   & - \\
\cmidrule{3-12}          &       & T-SANS & \textbf{54.8 } & 0.2   & \textbf{46.4 } & 0.3   & 60.1  & 0.1   & \textbf{69.6 } & 0.3   & 0.05 \\
\cmidrule{2-12}          & \multirow{2.2}[6]{*}{Uniq} & NS    & 45.2  & 0.1   & 34.3  & 0.1   & 51.1  & 0.1   & 65.8  & 0.3   & - \\
\cmidrule{3-12}          &       & SANS  & $^{\dagger}${\textbf{55.2 }} & 0.3   & $^{\dagger}${\textbf{46.8 }} & 0.5   & $^{\dagger}${\textbf{60.5 }} & 0.2   & $^{\dagger}${\textbf{70.0 }} & 0.3   & - \\
\cmidrule{3-12}          &       & T-SANS & 55.1  & 0.2   & $^{\dagger}${\textbf{46.8 }} & 0.3   & 60.3  & 0.1   & 69.9  & 0.2   & -0.1 \\
    \bottomrule
    \end{tabular}}
    }%
\end{table}%


==> inputs/dataset_for_analysis.tex <==
% after rebuttal
\begin{table}[t]
    \centering
    \small
    \caption{Statistics of the filtered sparser datasets.}
    % \resizebox{.95\columnwidth}{!}{	
    \begin{tabular}{ccrrrr}
    \toprule
    Dataset & Split & \multicolumn{1}{l}{Tuple} & \multicolumn{1}{l}{Query} & \multicolumn{1}{l}{Entity} & \multicolumn{1}{l}{Relation} \\
    \midrule
    \multirow{4}[6]{*}{FB15k-237-HL} & Total & 111,631 & 63,330 & 11,828 & 155 \\
\cmidrule{2-6}          & \#Train & 95,244 & 55,923 & 11,600 & 155 \\
\cmidrule{2-6}          & \#Valid & 7,571 & 6,918 & 4,933 & 90 \\
\cmidrule{2-6}          & \#Test & 8,816 & 7,830 & 5,406 & 89 \\
    \midrule
    \multirow{4}[6]{*}{WN18RR-HL} & Total & 14,697 & 14,675 & 12,973 & 10 \\
\cmidrule{2-6}          & \#Train & 13,758 & 13,785 & 12,275 & 10 \\
\cmidrule{2-6}          & \#Valid & 465   & 619   & 613   & 9 \\
\cmidrule{2-6}          & \#Test & 474   & 623   & 619   & 8 \\
    \midrule
    \multirow{4}[6]{*}{YAGO3-10-HL} & Total & 366,079 & 182,274 & 95,788 & 29 \\
\cmidrule{2-6}          & \#Train & 362,728 & 181,196 & 95,432 & 29 \\
\cmidrule{2-6}          & \#Valid & 1,662 & 2,316 & 2,113 & 13 \\
\cmidrule{2-6}          & \#Test & 1,689 & 2,359 & 2,135 & 14 \\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:artificial_datasets}
\end{table}


==> inputs/distribution.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/sum_query_frequency.png}
    \caption{Observed query frequencies summed from head-batch and tail-batch in training data of common datasets FB15k-237, WN18RR, and YAGO3-10, and artificial datasets FB15k-237-e, WN18RR-e, and YAGO3-10-e, respectively. Sorted from high to low\footnotemark.}
    \label{fig:query_freq}
\end{figure*}

\footnotetext{Note that both the x-axis and y-axis here are in logarithmic scale. If we use a normal scale, the long-tail feature will be more prominent.}



==> inputs/ratio.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/ratio.pdf}
    \caption{Total number of tuples, queries, entities, and relations represented in percentage for datasets FB15k-237, WN18RR, YAGO3-10, FB15k-237-e, WN18RR-e, and YAGO3-10-e.}
    \label{fig:aver_freq}
\end{figure}

==> inputs/segmented_tests.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/segmented_tests.pdf}
    \caption{Test results on the segmented test set\footnotemark of KGE model HAKE and RotatE on datasets FB15k-237, WN18RR, and YAGO3-10. Sorted using query frequency from high to low. $0.0\sim0.1$ means the targeted queries have the highest 10\% frequencies in the training data, and so on. As a comparison, the dotted lines indicate the test results on the whole test set for each model and each dataset.}
    \label{fig:segmented_tests}
\end{figure*}

\footnotetext{The segmented test set is made by sorting and selecting the queries in a certain frequency range in the training data, and composed by the tuples related to those queries in the whole test data. Each segmented test set has a 10\% number of targeted queries in the total queries of the training data.}

==> inputs/unified_loss_functions.tex <==
\begin{figure*}[t]
    \centering
    %\includegraphics[width=1\textwidth]{figures/unified_loss_functions_bar.pdf}
    \includegraphics[width=1\textwidth]{figures/unified_loss_functions_hbar.pdf}
    \includegraphics[width=1\textwidth]{figures/unified_loss_functions_hbar1.pdf}
    \includegraphics[width=1\textwidth]{figures/unified_loss_functions_hbar2.pdf}
    \caption{Performances of KGE models HAKE, RotatE, TransE, ComplEx, and DistMult on datasets FB15k-237, WN18RR, and YAGO3-10 using NS, SANS, UANS, and UANS$_p$ loss with subsampling settings (noted as \textit{Base, Freq, Uniq}) compared with non-subsampling setting (noted as \textit{None}).}
    \label{fig:unified_loss}
\end{figure*}
